Improving the convergence of SGD through adaptive batch sizes

Mini-batch stochastic gradient descent (SGD) and variants thereof approximate the objective function's gradient with a small number of training examples, aka the batch size. Small batch sizes require little computation for each model update but can yield high-variance gradient estimates, which poses some challenges for optimization. Conversely, large batches require more computation but can yield higher precision gradient estimates. This work presents a method to adapt the batch size to the model's training loss. For various function classes, we show that our method requires the same order of model updates as gradient descent while requiring the same order of gradient computations as SGD. This method requires evaluating the model's loss on the entire dataset every model update. However, the required computation is greatly reduced by approximating the training loss. We provide experiments that illustrate our methods require fewer model updates without increasing the total amount of computation.

==> src/fig-cifar.tex <==

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/cifar-mu}
        \caption{The number of model updates ($u$) vs. test accuracy.}
        \label{fig:cifar-test-updates}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/cifar-epochs}
        \caption{The number of epochs vs. test accuracy.}
        \label{fig:cifar-train-epochs}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/cifar-bs}
        \caption{How the batch sizes changes with model updates.}
        \label{fig:cifar-batch-size}
    \end{subfigure}
    \caption{%
        Different performance metrics for \PadaDamp, GeoDamp and GeoDamp LR on the CIFAR-10 dataset. Details are in Section~\ref{sec:cifar10}.
    }\label{fig:exp-cifar}
\end{figure*}


==> src/fig-padadamp-hsgd.tex <==

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/hsgd/padadamp-mu}
        \caption{How test accuracy varies with the number of model updates.\\}
        \label{fig:padadamp-hsgd-test-updates}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/hsgd/padadamp-epochs.pdf}
        \caption{How test accuracy varies with the number of epochs. GD requires 32,100 epochs to reach 75\% accuracy.}
        \label{fig:padadamp-hsgd-train-epochs}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/hsgd/padadamp-bs}
        \caption{How the batch size varies with the number of model updates.\\}
        \label{fig:padadamp-hsgd-batch-size}
    \end{subfigure}
    \caption{%
        Various performance metrics for the experiment in
        Section~\ref{sec:padadamp} with two additional optimizers to adapt HSGD
        to maximum batch sizes. Gradient descent (GD) requires 32,100 epochs to
        reach 75\% accuracy; correspondingly, the x-axis in
        Figure~\ref{fig:padadamp-hsgd-train-epochs} is trimmed.
``HSGD-1'' and ``HSGD-2'' decay the learning rate like $\bigO{1/k}$ and
$\bigO{1/k^2}$ respectively after the maximum batch size is reached.
    }\label{fig:padadamp-hsgd}
\end{figure*}


==> src/fig-padadamp.tex <==

\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/padadamp-mu}
        \caption{How test accuracy varies with the number of model updates.\\}
        \label{fig:padadamp-test-updates}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/padadamp-epochs.pdf}
        \caption{How test accuracy varies with the number of epochs.\\}
        \label{fig:padadamp-train-epochs}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[height=0.18\textheight]{figs/padadamp-bs}
        \caption{How the batch size varies with the number of model updates.\\}
        \label{fig:padadamp-batch-size}
    \end{subfigure}
    \caption{%
        Various performance metrics for the experiment in
        Section~\ref{sec:padadamp}. The legend in Figure~\ref{fig:padadamp-train-epochs} is shared with Figure~\ref{fig:padadamp-test-updates} and~\ref{fig:padadamp-batch-size}. Gradient descent (GD) requires 32,100 epochs to reach 75\% accuracy; correspondingly, the x-axis in
        Figure~\ref{fig:padadamp-train-epochs} is trimmed.
    }\label{fig:exp-padadamp}
    \vspace{-1em}
\end{figure*}

